A Practical Guide to the Partition Function of Atoms and Ions

The partition function, $U$, the number of available states in an atom or molecules, is crucial for understanding the physical state of any astrophysical system in thermodynamic equilibrium. There are surprisingly few {\em useful} discussions of the partition function's numerical value. Textbooks often define $U$; some give tables of representative values, while others do a deep dive into the theory of a dense plasma. Most say that it depends on temperature, atomic structure, density, and that it diverges, that is, it goes to infinity, at high temperatures, but few give practical examples. We aim to rectify this. We show that there are two limits, one and two-electron (or closed-shell) systems like H or He, and species with a complicated electronic structure like C, N, O, and Fe. The high-temperature divergence does not occur for one and two-electron systems in practical situations since, at high temperatures, species are collisionally ionized to higher ionization stages and are not abundant. The partition function is then close to the statistical weight of the ground state. There is no such simplification for many-electron species. $U$ is temperature-sensitive across the range of temperatures where an ion is abundant but remains finite at even the highest practical temperatures. The actual value depends on highly uncertain truncation theories in high-density plasmas. We show that there are various theories for continuum lowering but that they are not in good agreement. This remains a long-standing unsolved problem.

==> LocalMacros.tex <==
% put new macros in this file for eventual export to master file


==> macros.tex <==
% some names we use
\newcommand{\Cloudy}{\textsc{Cloudy}}
\newcommand{\Hazy}{\textsc{Hazy}}
\newcommand{\cdCommand}[1]{\textbf{#1}}
\newcommand{\cdVariable}[1]{\emph{#1}}
\newcommand{\cdSectionTitle}[1]{\emph{#1}}
\newcommand{\cdFilename}[1]{\texttt{#1}}
\newcommand{\cdRoutine}[1]{\emph{#1}}
\newcommand{\cdTerm}[1]{\textbf{\emph{#1}}}
\newcommand{\cdMono}[1]{\texttt{#1}}
\newcommand{\fixit}[1]{\textbf{FIXIT: #1}}
\font\manual=manfnt at 7pt \def\dbend{\hbox{\raise0.9ex\hbox{\manual\char127\hspace{0.6em}}}}
\newcommand{\experimental}{\texorpdfstring{\dbend}{??}}

% or symbol provided by Will H
\newcommand\OR{\texorpdfstring{\ensuremath{\vert}}{|}}

% Matt's 1.23\e{-2} 
\providecommand{\e}[1]{\ensuremath{\times 10^{#1}}}


% \ion from Will, replace AAS version
\newcommand\Ion[2]{\ensuremath{\mathrm{#1\,\scriptstyle #2}}}

% macro sometimes found in ADS bibtex entries
\newcommand{\mdash}{---} 

% ion is in the aas style
\newcounter{INTERNALionstage}
\providecommand{\ion}[2]{% replace the aastex version
  \setcounter{INTERNALionstage}{#2}%
  \Ion{#1}{\Roman{INTERNALionstage}}}

\providecommand{\red}[1]{{\color{red}#1}}

% Will's todo and done macros
%\newcommand\TODO[1]{\textbf{\boldmath [#1]}}
\newcommand{\TODO}[1]{\textcolor{red}{{\textbf{\boldmath [#1]}}}}
\newcommand\DONE[1]{{\color{green!50!gray} \textbf{DONE}} {\color{white!80!black!80!green} #1}}

\newcommand{\Av}{A$_{\rm V}$}

\def\gtsim{\mathrel{\hbox{\rlap{\hbox{\lower4pt\hbox{$\sim$}}}\hbox{$>$}}}}
\def\lesssim{\mathrel{\hbox{\rlap{\hbox{\lower4pt\hbox{$\sim$}}}\hbox{$<$}}}}
\def\Msunpyr{M$_{\odot}\,$yr$^{-1}$}
\def\Msun{M$_{\odot}$}
%       Based on PATs UNITS.TEX with some additions
%
%       Simple units
%
\def\A{{\rm\thinspace \AA}}
\def\cm{{\rm\thinspace cm}}
\def\as{{\rm\thinspace arcsec}}
\def\erg{{\rm\thinspace erg}}
\def\eV{{\rm\thinspace eV}}
\def\g{{\rm\thinspace g}}
\def\ga{{\rm\thinspace gauss}}
\def\hr{{\rm\thinspace hr}}
\def\Hz{{\rm\thinspace Hz}}
\def\K{{\rm\thinspace K}}
\def\keV{{\rm\thinspace keV}}
\def\km{{\rm\thinspace km}}
\def\kpc{{\rm\thinspace kpc}}
\def\Lsun{\mbox{$\rm\thinspace L_{\odot}$}}
\def\m{{\rm\thinspace m}}
\def\MeV{{\rm\thinspace MeV}}
\def\mJy{{\rm\thinspace mJy}}
\def\micron{\hbox{$\mu$m}}
\def\Mpc{{\rm\thinspace Mpc}}
\def\Msun{\mbox{$\rm\thinspace M_{\odot}$}}
\def\nm{{\rm\thinspace nm}}
\def\pc{{\rm\thinspace pc}}
\def\ps{{\rm\thinspace s^{-1}}}
\def\pcc{{\rm\thinspace cm^{-3}}}
\def\Ryd{{\rm\thinspace Ryd}}
\def\s{{\rm\thinspace s}}
\def\sr{{\rm\thinspace sr}}
\def\W{{\rm\thinspace W}}
\def\yr{{\rm\thinspace yr}}
%
%       Compound units
%
\def\keVscm{\mbox{$\keV\cm^{2}\,$}}
\def\cmps{\mbox{$\cm\s^{-1}\,$}}
\def\cmpss{\mbox{$\cm\s^{-2}\,$}}
\def\ccmps{\mbox{$\cm^{3}\s^{-1}\,$}}
\def\ergpccmps{\mbox{$\erg\cm^{-3}\s^{-1}\,$}}
\def\ergpg{\mbox{$\erg\g^{-1}\,$}}
\def\ergpscm{\mbox{$\erg\cm^{-2}\,$}}
\def\ergpscmps{\mbox{$\erg\cm^{-2}\s^{-1}\,$}}
\def\ergpscmpspsas{\mbox{$\erg\cm^{-2}\s^{-1}\as^{-2}\,$}}
\def\ergpscmpspa{\mbox{$\erg\cm^{-2}\s^{-1}\A^{-1}\,$}}
\def\ergps{\mbox{$\erg\s^{-1}\,$}}
\def\gpcm{\mbox{$\g\cm^{-3}\,$}}
\def\gpcmps{\mbox{$\g\cm^{-3}\s^{-1}\,$}}
\def\gps{\mbox{$\g\s^{-1}\,$}}
\def\uJy{\mbox{$\mu${\rm Jy}}}
\def\kmps{\mbox{$\km\ps\,$}}
\def\kmpspMpc{\mbox{$\kmps\Mpc^{-1}\,$}}
\def\Lsunppc{\mbox{$\Lsun\pc^{-3}\,$}}
\def\Msunpc{\mbox{$\Msun\pc^{-3}\,$}}
\def\Msunpkpc{\mbox{$\Msun\kpc^{-1}\,$}}
\def\Msunppc{\mbox{$\Msun\pc^{-3}\,$}}
\def\Msunppcpyr{\mbox{$\Msun\pc^{-3}\yr^{-1}\,$}}
\def\Msunpyr{\mbox{$\Msun\yr^{-1}\,$}}
\def\Msunpyrpkpc{\mbox{$\Msun\yr^{-1}\kpc^{-1}\,$}}
\def\ps{\mbox{$\s^{-1}\,$}}
\def\pscm{\mbox{$\cm^{-2}\,$}}
\def\psm{\mbox{$\m^{-2}\,$}}
\def\pccm{\mbox{$\cm^{-3}\,$}}
\def\pscm{\mbox{$\cm^{-2}\,$}}
\def\pscmps{\mbox{$\cm^{-2}\, \s^{-1}\,$}}
\def\pcm{\mbox{$\m^{-3}\,$}}
\def\pccmK{\mbox{$\cm^{-3}\K$}}
\def\pcmK{\mbox{$\m^{-3}\K$}}
\def\pressure{\mbox{$\g\, \cm^{-1}\, \s^{-2}\,$}}
\def\pyr{\mbox{$\yr^{-1}\,$}}
\def\pyrppc{\mbox{$\yr^{-1}\pc^{-1}\,$}}
\def\scm{\mbox{$\cm^{2}\,$}}
\def\Wpsm{\mbox{$\W\psm\,$}}
\def\Wpscm{\mbox{$\W\pscm\,$}}
\def\WHz{\mbox{$\W\Hz\,$}}
%
% spectral lines
%
\def\la{\mbox{{\rm L}$\alpha$}}
\def\pa{\mbox{{\rm P}$\alpha$}}
\def\ha{\mbox{{\rm H}$\alpha$}}
\def\hb{\mbox{{\rm H}$\beta$}}
\def\hi{\mbox{{\rm H~{\sc i}}}}
\def\hii{\mbox{{\rm H~{\sc ii}}}}
\def\hei{\mbox{{\rm He~{\sc i}}}}
\def\heii{\mbox{{\rm He~{\sc ii}}}}
\def\ci{\mbox{{\rm C~{\sc i}}}}
\def\cii{\mbox{{\rm C~{\sc ii}}}}
\def\ciii{\mbox{{\rm C~{\sc iii}}}}
\def\civ{\mbox{{\rm C~{\sc iv}}}}
\def\ni{\mbox{{\rm N~{\sc i}}}}
\def\nii{\mbox{{\rm N~{\sc ii}}}}
\def\oi{\mbox{{\rm O~{\sc i}}}}
\def\oii{\mbox{{\rm O~{\sc ii}}}}
\def\oiii{\mbox{{\rm O~{\sc iii}}}}
\def\neii{\mbox{{\rm Ne~{\sc ii}}}}
\def\neiii{\mbox{{\rm Ne~{\sc iii}}}}
\def\nev{\mbox{{\rm Ne~{\sc v}}}}
\def\mgii{\mbox{{\rm Mg~{\sc ii}}}}
\def\cliii{\mbox{{\rm Cl~{\sc iii}}}}
\def\sii{\mbox{{\rm S~{\sc ii}}}}
\def\siii{\mbox{{\rm S~{\sc iii}}}}
\def\ariii{\mbox{{\rm Ar~{\sc iii}}}}
\def\caii{\mbox{{\rm Ca~{\sc ii}}}}
\def\fei{\mbox{{\rm Fe~{\sc i}}}}
\def\feii{\mbox{{\rm Fe~{\sc ii}}}}
\def\feiii{\mbox{{\rm Fe~{\sc iii}}}}
\def\feiv{\mbox{{\rm Fe~{\sc iv}}}}
\def\fev{\mbox{{\rm Fe~{\sc v}}}}
\def\fevi{\mbox{{\rm Fe~{\sc vi}}}}
\def\fevii{\mbox{{\rm Fe~{\sc vii}}}}
\def\feviii{\mbox{{\rm Fe~{\sc viii}}}}
\def\feix{\mbox{{\rm Fe~{\sc ix}}}}
\def\fex{\mbox{{\rm Fe~{\sc x}}}}
\def\fexi{\mbox{{\rm Fe~{\sc xi}}}}
\def\fexii{\mbox{{\rm Fe~{\sc xii}}}}
\def\fexiii{\mbox{{\rm Fe~{\sc xiii}}}}
\def\fexiv{\mbox{{\rm Fe~{\sc xiv}}}}
\def\fexv{\mbox{{\rm Fe~{\sc xv}}}}
\def\fexvi{\mbox{{\rm Fe~{\sc xvi}}}}
\def\fexvii{\mbox{{\rm Fe~{\sc xvii}}}}
\def\fexviii{\mbox{{\rm Fe~{\sc xviii}}}}
\def\fexix{\mbox{{\rm Fe~{\sc xix}}}}
\def\fexx{\mbox{{\rm Fe~{\sc xx}}}}
\def\fexxi{\mbox{{\rm Fe~{\sc xxi}}}}
\def\fexxii{\mbox{{\rm Fe~{\sc xxii}}}}
\def\fexxiii{\mbox{{\rm Fe~{\sc xxiii}}}}
\def\fexxiv{\mbox{{\rm Fe~{\sc xxiv}}}}
\def\fexxv{\mbox{{\rm Fe~{\sc xxv}}}}
\def\fexxvi{\mbox{{\rm Fe~{\sc xxvi}}}}
%
% types of baryons
\def\water{\mbox{{\rm H}$_2${\rm O}}}
\def\CO{\mbox{{\rm CO}}}
\def\OH{\mbox{{\rm OH}}}
\def\htwo{\mbox{{\rm H}$_2$}}
\def\hone{\mbox{{\rm H}$^0$}}
\def\h0{\mbox{{\rm H}$^0$}}
%
% \def\H{\mbox{{\rm H}}}
%
\def\hplus{\mbox{{\rm H}$^+$}}
\def\hminus{\mbox{{\rm H}$^-$}}
% cannot have numbers in names, so cap Oh represents zero
\def\hO{\mbox{{\rm H}$^0$}}
\def\heO{\mbox{{\rm He}$^0$}}
\def\heo{\mbox{{\rm He}$^0$}}
\def\heplus{\mbox{{\rm He}$^+$}}
\def\hePP{\mbox{{\rm He}$^{2+}$}}
\def\cO{\mbox{{\rm C}$^0$}}
\def\cplus{\mbox{{\rm C}$^+$}}
%
\def\Hrec{\mbox{${\rm H}_{rec}$}}
%\def\Hrec{\mbox{$H_{rec}$}}
\def\centreline{\centerline}
%
% Nina
\DeclareMathAlphabet{\vib}{OML}{cmm}{m}{it}
% From Glenn
\newcommand*{\satellite}[1]{\textit{#1}}
\newcommand*{\xmm}{\satellite{XMM-Newton}}
\newcommand*{\chandra}{\satellite{Chandra}}
\newcommand*{\asca}{\satellite{ASCA}}
\newcommand*{\rosat}{\satellite{ROSAT}}
\newcommand*{\prog}[1]{\textsc{#1}}
%% For kb, mH. etc. Italic with non-italic subscript.
\newcommand*{\mysub}[2]{\ensuremath{#1_{\mathrm{#2}}}}

